Identification of $dq$-Asymmetric Impedances as Complex Transfer Functions Using a Single Arbitrary Excitation

Cross-coupling between the $dq$ coordinates makes the identification of asymmetric grid impedances a challenging problem, particularly near the fundamental frequency where the asymmetric coupling is strongest. Existing schemes usually handle it either by perturbing the two coordinates sequentially, which lengthens the measurement, or by using a time-domain method with a global parametric model whose order must be tuned. This paper develops a single-shot active non-parametric frequency-domain method that avoids both. The equivalent impedance is parameterized by a pair of single-input single-output complex transfer functions. Each spectral line is fitted with a local rational model; the leakage and transient contributions are estimated, so that neither periodic steady-state excitation nor repeated excitation cycles are required. We give the exact finite-time discrete Fourier transform relation for the conjugate-coupled complex-signal model, and analyse the distortion that a stationary-frame filter placed ahead of the Park transform imposes on the identified pair. The method is validated on a controller hardware-in-the-loop platform against an analytically derived small-signal model, for a symmetric grid and for the same grid with an added grid-following converter that renders it asymmetric. Both complex transfer functions and all four real transfer functions of the $dq$ impedance are recovered over a wide band from a single one-second record of a random excitation, at 1 Hz resolution.

==> config/macros.tex <==
\makeatletter
\newcommand{\pushright}[1]{\ifmeasuring@#1\else\omit\hfill$\displaystyle#1$\fi\ignorespaces}
\newcommand{\pushleft}[1]{\ifmeasuring@#1\else\omit$\displaystyle#1$\hfill\fi\ignorespaces}
\makeatother

\providecommand{\eu}{\ensuremath{\mathrm{e}}}

\makeatletter
\providecommand*{\diff}%
{\@ifnextchar^{\DIfF}{\DIfF^{}}}
\def\DIfF^#1{%
\mathop{\mathrm{\mathstrut d}}%
\nolimits^{#1}\gobblespace}
\def\gobblespace{%
\futurelet\diffarg\opspace}
\def\opspace{%
\let\DiffSpace\!%
\ifx\diffarg(%
\let\DiffSpace\relax
\else
\ifx\diffarg[%
\let\DiffSpace\relax
\else
\ifx\diffarg\{%
\let\DiffSpace\relax
\fi\fi\fi\DiffSpace}


\providecommand*{\deriv}[3][]{%
\frac{\diff^{#1}#2}{\diff #3^{#1}}}

\newcommand{\vc}{\mathrm{vec}}
\newcommand{\paren}[1]{\ensuremath{\left( #1\right)}}
\newcommand{\sparen}[1]{\ensuremath{(#1)}}
\newcommand{\clint}[1]{\ensuremath{\left[ #1\right]}}
\newcommand{\set}[1]{\ensuremath{\left\{ #1\right\}}}
\newcommand{\matr}[1]{\ensuremath{\begin{bmatrix} #1 \end{bmatrix}}}
\newcommand{\norm}[1]{\ensuremath{\left\| #1\right\|}}
\newcommand{\snorm}[1]{\ensuremath{\| #1\|}}
\newcommand{\abs}[1]{\ensuremath{\left| #1\right|}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\naturals}{\mathbb{N}}
\newcommand{\opnorm}[1]{\ensuremath{\| #1\|_{\mathrm{op}}}}
\newcommand{\hsnorm}[1]{\ensuremath{\| #1\|_{\mathrm{F}}}}
\newcommand{\hinfnorm}[1]{\ensuremath{\| #1\|_{\mathcal{H}_{\infty}}}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\toep}{\mathcal{T}}
\newcommand{\cconv}{\circledast}
\newcommand{\conv}{*}
\renewcommand{\Pr}{\mathbb{P}}

\newcommand{\du}{d_{{u}}}
\newcommand{\Du}{D_{{u}}}
\newcommand{\cu}{c_{{u}}}
\newcommand{\sigmau}{\sigma_{{u}}}
\newcommand{\sigmae}{\sigma_{{e}}}
\newcommand{\dy}{d_{{y}}}
\newcommand{\de}{d_{{e}}}
\newcommand{\Np}{N_p}
\newcommand{\Ntot}{N_\mathrm{tot}}
\newcommand{\cplx}{\mathbb{C}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\blkdiag}{\mathrm{blkdiag}}
\newcommand{\p}{\mathrm{\mathstrut p}}
\newcommand{\A}{\mathcal{A}}


\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\bi}{\boldsymbol{i}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bg}{\boldsymbol{g}}
\newcommand{\bI}{\boldsymbol{I}}
\newcommand{\bV}{\boldsymbol{V}}
\newcommand{\bG}{\boldsymbol{G}}
\newcommand{\bT}{\boldsymbol{T}}
\newcommand{\bU}{\boldsymbol{U}}
\newcommand{\bY}{\boldsymbol{Y}}
\newcommand{\bA}{\boldsymbol{A}}
\newcommand{\bB}{\boldsymbol{B}}
\newcommand{\bC}{\boldsymbol{C}}
\newcommand{\bE}{\boldsymbol{E}}
\newcommand{\bEps}{\boldsymbol{\mathcal{E}}}
\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\1}{\boldsymbol{1}}


\newcommand{\F}{\mathcal{F}}



% for the square hat used in the Appendix
% requires the package: stackengine
\def\rlwd{.4pt}
\def\rlht{1.1pt}
\def\shatvrule{\rule{\rlwd}{\rlht}}
\def\shat#1{%
  \setbox0=\hbox{$#1$}%
  \stackon[0pt]{\stackon[1pt]{\ensuremath{#1}}{%
    \shatvrule\kern\wd0\kern-\rlwd\kern-\rlwd\shatvrule}}%
    {\rule{\wd0}{\rlwd}}%
}

%=====================================================================
%  Additions for the journal version
%=====================================================================
\newcommand{\Gp}{\bG_{+}}
\newcommand{\Gm}{\bG_{-}}
\newcommand{\creflect}[1]{#1^{\ast}}   % conjugate reflection F^*(s) := [F(s^*)]^*
\newcommand{\wg}{\omega_g}
\newcommand{\Hup}{H_{+}}
\newcommand{\Hlo}{H_{-}}
\newcommand{\degop}{\operatorname{deg}}
\newcommand{\sigmax}{\bar{\sigma}}


%=====================================================================
%  Path fragments for the one-line diagrams (same visual style as the
%  conference figure: hand-drawn IEC zig-zag resistors, IEC inductors)
%=====================================================================
% horizontal resistor with straight leads, total length 1.45
\newcommand{\resH}{-- ++(0.20,0) -- ++(0.10,-0.15) -- ++(0.10,0.33)
                   -- ++(0.20,-0.33) -- ++(0.10,0.33) -- ++(0.20,-0.33)
                   -- ++(0.10,0.33) -- ++(0.20,-0.33) -- ++(0.05,0.15)
                   -- ++(0.20,0)}
% vertical resistor with straight leads, total drop 1.45
\newcommand{\resV}{-- ++(0,-0.20) -- ++(-0.15,-0.10) -- ++(0.33,-0.10)
                   -- ++(-0.33,-0.20) -- ++(0.33,-0.10) -- ++(-0.33,-0.20)
                   -- ++(0.33,-0.10) -- ++(-0.33,-0.20) -- ++(0.15,-0.05)
                   -- ++(0,-0.20)}
% shunt capacitor to ground, hanging from (#1,#2)
\newcommand{\shuntcap}[2]{%
  \draw (#1,#2) -- (#1,#2-0.80);
  \draw (#1-0.30,#2-0.80) -- (#1+0.30,#2-0.80);
  \draw (#1-0.30,#2-0.95) -- (#1+0.30,#2-0.95);
  \draw (#1,#2-0.95) -- (#1,#2-1.45);
  \draw (#1-0.15,#2-1.45) -- (#1+0.15,#2-1.45);
  \draw (#1-0.08,#2-1.52) -- (#1+0.08,#2-1.52);}
% ground stub below (#1,#2)
\newcommand{\gnd}[2]{%
  \draw (#1-0.15,#2) -- (#1+0.15,#2);
  \draw (#1-0.08,#2-0.07) -- (#1+0.08,#2-0.07);}
% ideal AC source centred at (#1,#2)
\newcommand{\acsource}[2]{%
  \draw (#1,#2) circle (0.32);
  \draw plot[smooth,tension=.7] coordinates
    {(#1-0.20,#2-0.05) (#1-0.10,#2+0.15) (#1+0.10,#2-0.15) (#1+0.20,#2+0.05)};}


==> figures/fig_ratio1.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[hilaxis, width=1.02\columnwidth, height=4.0cm,
             xmin=-1000, xmax=1000, xtick={-1000,-500,0,500,1000},
             ymin=-75, ymax=0, ytick={0,-20,-40,-60},
             xlabel={Frequency [\si{\Hz}]}, ylabel={$r(\omega)$ [\si{\dB}]}]
\addplot[truecurve] table[x=f,y=r_dB] {figures/data/case2_ratio_true.dat};
\end{axis}
\end{tikzpicture}
\caption{Case~2: the ratio $r(\omega)=|\bG_-(j\omega)|/|\bG_+(j\omega)|$, which
measures how strong the mirror-frequency coupling is relative to the direct
term. The coupling is significant only in a narrow band around the
fundamental.}
\label{fig:ratio}
\end{figure}

